Joint Energy Efficient and QoS-aware Path Allocation and VNF Placement for Service Function Chaining

Service Function Chaining (SFC) allows the forwarding of a traffic flow along a chain of Virtual Network Functions (VNFs, e.g., IDS, firewall, and NAT). Software Defined Networking (SDN) solutions can be used to support SFC reducing the management complexity and the operational costs. One of the most critical issues for the service and network providers is the reduction of energy consumption, which should be achieved without impact to the quality of services. In this paper, we propose a novel resource (re)allocation architecture which enables energy-aware SFC for SDN-based networks. To this end, we model the problems of VNF placement, allocation of VNFs to flows, and flow routing as optimization problems. Thereafter, heuristic algorithms are proposed for the different optimization problems, in order find near-optimal solutions in acceptable times. The performance of the proposed algorithms are numerically evaluated over a real-world topology and various network traffic patterns. The results confirm that the proposed heuristic algorithms provide near optimal solutions while their execution time is applicable for real-life networks.

==> Nomenclature.tex <==
%\section{Nomenclature}\label{sez:4\part{title}}
\vspace{-5px}
%\vspace{8px}
	\mbox{}
	%\scriptsize{
		\footnotesize {
	\setlength{\nomlabelwidth}{2cm}
	\setlength{\nomitemsep}{-\parsep}
	\nomenclature[I]{Node}{Server}
	\nomenclature[I]{VM}{Virtual Machine}
	\nomenclature[I]{OF}{OpenFlow}
	\nomenclature[I]{OF Switch}{OpenFlow-enabled Switch}
	\nomenclature[I]{SFC}{Service Function Chaining}
	\nomenclature[I]{Service}{Service Function}
	\nomenclature[I]{RA}{Resource Allocation}
	\nomenclature[I]{RR}{Resource Reallocation}
		% Parameters
	%	\nomenclature[P]{$ST_{ji}$}{earliest starting time of task $i$ in home $j$}
	%	\nomenclature[P]{$ET_{ji}$}{latest finishing time of task $i$ in home $j$}
	    % Variabes
	%	\nomenclature[V]{$P_{ESS}(t)$}{electricity in energy storage system at time $t$ [$kW_e$]}
	\printnomenclature
}\vspace{-5px}
